Generative Neural Network Channel Modeling for Millimeter-Wave UAV Communication

The millimeter wave bands are being increasingly considered for wireless communication to unmanned aerial vehicles (UAVs). Critical to this undertaking are statistical channel models that describe the distribution of constituent parameters in scenarios of interest. This paper presents a general modeling methodology based on data-training a generative neural network. The proposed generative model has a two-stage structure that first predicts the link state (line-of-sight, non-line-of-sight, or outage), and subsequently feeds this state into a conditional variational autoencoder (VAE) that generates the path losses, delays, and angles of arrival and departure for all the propagation paths. The methodology is demonstrated for 28 GHz air-to-ground channels between UAVs and a cellular system in representative urban environments, with training datasets produced through ray tracing. The demonstration extends to both standard base stations (installed at street level and downtilted) as well as dedicated base stations (mounted on rooftops and uptilted). The proposed approach is able to capture complex statistical relations in the data and it significantly outperforms standard 3GPP models, even after refitting the parameters of those models to the data.

==> benchmark_3gpp_v1.tex <==

To complete the test-drive of the proposed generative model, it is fitting to benchmark it against the alternatives offered by existing standard models, namely 3GPP models and specifically their UMi-AV (urban micro with aerial vehicles) scenario.
The current UMi-AV model, with its parameters given by \gls{3gpp}, does not accurately capture the complex environments in question. 

In order to provide a fair benchmark for our proposed two-stage architecture, we will perform a re-parameterization.
This process consists of first determining what constant parameters characterize the UMi-AV channel model, then finding new values for those constants that allow the model to best describe the multi-path components of each city. 
Critically, a new set of parameters will be determined for each city, allowing for maximum flexibility of the formerly generalized standard model.

%\angel{Let's indicate that, for the path loss at least, we're extrapolating a sub-6 GHz model.}
%\angel{William, let's explain here what we're going to do in this section, so the term "re-parameterization" doesn't hit the reader as a surprise when it appears.}


\subsection{LOS Probability}
\label{subsubsec:3gpp_los}

We first examine the probability of \gls{los}, $P_{\rm LOS}$.
The 3GPP model takes in several parameters such as the heights of the receiver and transmitter, as well as their horizontal distance, $d_{\rm 2D}$ \cite{3GPP38901}. 
If the \gls{uav} height $h_{UT}$ is between \SI{1.5}{\meter} and \SI{22.5}{\meter}, then 
\begin{equation}
    P_{\rm LOS} = 
    \begin{cases}
        1 & d_{\rm 2D} \leq \alpha_1 \\
        \frac{\alpha_1}{d_{\rm 2D}}+e^{-\frac{d_{\rm 2D}}{\alpha_2}}\left( 1-\frac{\alpha_1}{d_{\rm 2D}}\right) & \alpha_1 \leq d_{\rm 2D}
    \end{cases} 
    \label{eq:plos_low}
\end{equation}
whereas, if $h_{UT}>$ \SI{22.5}{\meter},
\begin{equation}
    P_{\rm LOS} = 
    \begin{cases}
        1 & d_{\rm 2D} \leq d_1 \\
        \frac{d_1}{d_{\rm 2D}} + e^{-\frac{d_{\rm 2D}}{p_1}}\left( 1 - \frac{d_1}{d_{\rm 2D}}\right) & d_{\rm 2D} > d_1
    \end{cases}
    \label{eq:plos_high}
\end{equation}
where
\begin{equation}
\begin{split}
    & p_1 = \alpha_3\log_{10}(h_{UT})+\alpha_4 \\
    & d_1 = \max(\alpha_5\log_{10}(h_{UT})+\alpha_6,\alpha_1) .
\end{split}
\label{eq:plos_vars}
\end{equation}
This is a parameterization of the standard model yielding the vector of six variables which we will learn for each individual city to compute the probability of \gls{los}: $\bm{\alpha} = [\alpha_1, \alpha_2, \alpha_3, \alpha_4, \alpha_5, \alpha_6]$.
The nominal parameters given by the \gls{3gpp} UMi-AV model are 
\begin{equation}
    \bm{\alpha}_{nom} = [18, 36, 294.05, -432.94, 233.98, -0.95]
\end{equation}
with the first two parameters characterizing (\ref{eq:plos_low}), and the last four parameters needed in (\ref{eq:plos_high}) and (\ref{eq:plos_vars}).

\begin{table}
    %\vspace{1mm}
    \caption{3GPP Re-Parameterization NNs}
    \label{table:3gpp_nn_param}
    \centering
    \begin{tabular}{l|c|c|}
    \cline{2-3}
    {} &
    \shortstack{$P_{\rm LOS}$ NN} & \shortstack{Path Loss NN} \\ \hline
    \multicolumn{1}{|l|}{Number of inputs} &
    5 & 6 \\ \hline
    \multicolumn{1}{|l|}{Number of outputs} &
    \multicolumn{2}{c|}{1} \\ \hline
    \multicolumn{1}{|l|}{Optimizer} &
    \multicolumn{2}{c|}{Adam} \\ \hline
    \multicolumn{1}{|l|}{Loss Function} &
    Binary Cross Entropy & Mean-Squared Error \\ \hline
    \multicolumn{1}{|l|}{Learning rate} &
    \multicolumn{2}{c|}{$10^{-3}$} \\ \hline
    \multicolumn{1}{|l|}{Epochs} &
    \multicolumn{2}{c|}{50} \\ \hline
    \multicolumn{1}{|l|}{Batch size} &
    \multicolumn{2}{c|}{128} \\ \hline
    \end{tabular}
\noindent
\end{table}
\begin{table*}[t!]
    \vspace{1mm}
    \caption{$P_{LOS}$: Mean Absolute Error}
    \label{tab:plos_error}
    \centering
    \begin{tabular}{l|c|c|c|c|c|}
    \cline{2-6}
    {}
    & \shortstack{Tokyo, Japan} 
    & \shortstack{Beijing, China} 
    & \shortstack{London, UK} 
    & \shortstack{Moscow, Russia}
    & \shortstack{Boston, USA} \\ \hline
    \multicolumn{1}{|l|}{Default 3GPP Model}
    & \cellcolor{red!25}0.272 & \cellcolor{red!25}0.247 & \cellcolor{red!25}0.303 & \cellcolor{red!25}0.180 & \cellcolor{red!25}0.336 \\ \hline
    \multicolumn{1}{|l|}{Re-parameterized 3GPP Model}
    & 0.040 & \cellcolor{green!25}0.056 & \cellcolor{green!25}0.057 & 0.058 & 0.047\\ \hline
    \multicolumn{1}{|l|}{Proposed Generative Model}
    & \cellcolor{green!25}0.036 & 0.058 & \cellcolor{green!25}0.057 & \cellcolor{green!25}0.034 & \cellcolor{green!25}0.041\\ \hline
    \end{tabular}
\noindent
\end{table*}

\begin{table*}[b!]
    \vspace{1mm}
    \caption{Path Loss: Mean Absolute Error}
    \label{tab:pl_error}
    \centering
    \begin{tabular}{l|c|c|c|c|c|}
    \cline{2-6}
    {}
    & \shortstack{Tokyo, Japan} 
    & \shortstack{Beijing, China} 
    & \shortstack{London, UK} 
    & \shortstack{Moscow, Russia}
    & \shortstack{Boston, USA} \\ \hline
    \multicolumn{1}{|l|}{Default 3GPP Model}
    & \cellcolor{red!25}0.0392 & \cellcolor{red!25}0.0412 & \cellcolor{red!25}0.0398 & \cellcolor{red!25}0.0388 & \cellcolor{red!25}0.0414 \\ \hline
    \multicolumn{1}{|l|}{Re-parameterized 3GPP Model}
    & 0.0308 & 0.0339 & 0.0328 & 0.0332 & 0.0352\\ \hline
    \multicolumn{1}{|l|}{Proposed Generative Model}
    & \cellcolor{green!25}0.0131 & \cellcolor{green!25}0.0093 & \cellcolor{green!25}0.0110 & \cellcolor{green!25}0.0079 & \cellcolor{green!25}0.0129\\ \hline
    \end{tabular}
\noindent
\end{table*}


Following this parameterization, we design a NN with weights $\mathbf{w}_i$ which serve as multipliers to the nominal parameters $\bm{\alpha}_{nom}$ to obtain the final parameters used to compute $P_{LOS}$.
%\angel{This is rather confusing. We have defined $\mathbf{p}_{nom}$ as the "vector of nominal parameters", and here we refer to $\mathbf{x}_0$ as the "nominal parameters". Even I'm getting lost :-)}
%\william{Sorry, I tried to word this in a concise but understandable way. I'm trying to say that $\mathbf{w}$ are the weights of the neural network, and act as multipliers to the nominal parameters $\mathbf{p}_{nom}$. It is the element-wise product of $\mathbf{w}$ and $\mathbf{p}_{nom}$ (scaled nominal parameters) which are used to compute $P_{LOS}$.}.
The weights are updated during training with initial values of $\mathbf{w}_0 = [1,1,1,1,1,1]$. 
The NN uses a custom layer which implements (\ref{eq:plos_low}), (\ref{eq:plos_high}), and (\ref{eq:plos_vars}) to compute the $P_{LOS}$ using the network weights $\mathbf{w}_i$ and inputs
\begin{equation}
    \mathbf{x}_i = \left[\log_{10}(h_{UT}),d_{2D},h_{UT}, h_{gNB}\right]
\end{equation}
The NN, described in Table \ref{table:3gpp_nn_param}, is trained with data from each of the five cities in Fig.~\ref{fig:all_cities} to obtain a distinct set of parameters for each.
We also impose that the NN weights be restricted to the interval $[0.01,10]$ to prevent the model from overfitting, and to keep the final parameters close to the nominal parameters.

The results are displayed in Table \ref{tab:plos_error}, where the mean error over a grid of horizontal and vertical distances is computed for the default \gls{3gpp} model (nominal parameters), the re-parameterized \gls{3gpp} model, and our proposed generative model.
These results show that the structure of the \gls{3gpp} model for the probability of \gls{los} is well parameterized, and can be trained to generate link state samples that have very small error when compared to the data. 
In fact, for Beijing and London, the trained \gls{3gpp} model just narrowly outperforms our proposed model. 
Our proposed link-state predictor, however, has a lower error than even the trained \gls{3gpp} model for the majority of the cities, and with higher margins.

\subsection{Path Loss}
\label{subsubsec:3gpp_pl}

We employ a similar strategy to re-parameterize the standard \gls{3gpp} model for the path loss generation.
The path loss is computed according to equations given by Table B-1 in \cite{3GPP36777}.
It is important to realize here that unlike the case for computing $P_{LOS}$, which depends entirely on the geometry of the environment, the path loss is frequency dependent. 
As such, we proceed with the acknowledgement that the standard model structure and its parameters were originally derived from data measured at sub-\SI{6}{GHz} frequencies.
% Thus, we have path loss nominal parameters 
% \begin{equation}
% \begin{split}
%     & \bm{\alpha}_{nom,los} = [32.4, 21, 20, 32.4, 40, 20, -9.5, 30.9, 22.5, -0.5, 20] \\
%     & \bm{\alpha}_{nom,nlos} = [35.3, 22.4, 21.3, -0.3, 32.4, 43.2, -7.6, 20]
% \end{split}
% \end{equation}

Again, following a parameterization of the path loss equations of the standard model, another custom neural network layer is designed to compute the path loss following the \gls{3gpp} model structure.
The input includes the same parameters as the input used in the $P_{LOS}$ network, but now includes a predicted link state:
\begin{equation}
    \mathbf{x}_i = \left[\log_{10}(h_{UT}),d_{2D},h_{UT}, h_{gNB}, s\right]
\end{equation}
The neural network is configured and trained according to the parameters in Table~\ref{table:3gpp_nn_param}.
\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\columnwidth]{Figures/eval_3gpp_UAS_pathloss_tokyo.png}
    \caption{Path loss fitting for generative models in Tokyo, Japan.}
    \label{fig:model_compare_pl_tokyo}
\end{figure}
The results of this re-parameterization are shown by Table~\ref{tab:pl_error}, where the error between any given model and the data is computed by first using the model to generate samples based on the condition variables of the test dataset, and then computing the mean difference between the model and data CDFs. 
Unlike the probability of \gls{los} model discussed in Sec.~\ref{subsubsec:3gpp_los}, our proposed two-state generative model outperforms the re-parameterized \gls{3gpp} model significantly for all five cities that were studied. 

This is made clear by plotting the CDFs of path losses for the original Remcom data, the default (or nominal) \gls{3gpp} model, the re-parameterized \gls{3gpp} model, and our proposed \gls{vae} model for specifically the city of Tokyo in Fig.~\ref{fig:model_compare_pl_tokyo}.
While the path loss model generated by the trained \gls{3gpp} model indeed performs better than the default one, we can see that our proposed architecture is able to best approximate the distribution of the actual data.
This fact is true when comparing the generative schemes to the data of all five respective cities.
